MoTCoder: Elevating Large Language Models with Modular of Thought for Challenging Programming Tasks

Large Language Models (LLMs) have showcased impressive capabilities in handling straightforward programming tasks. However, their performance tends to falter when confronted with more challenging programming problems. We observe that conventional models often generate solutions as monolithic code blocks, restricting their effectiveness in tackling intricate questions. To overcome this limitation, we present Module-of-Thought Coder (MoTCoder). We introduce a framework for MoT instruction tuning, designed to promote the decomposition of tasks into logical sub-tasks and sub-modules. Our investigations reveal that, through the cultivation and utilization of sub-modules, MoTCoder significantly improves both the modularity and correctness of the generated solutions, leading to substantial pass@1 improvements of 5.9% on APPS and 5.8% on CodeContests. MoTCoder also achieved significant improvements in self-correction capabilities, surpassing the current SOTA by 3.3%. Additionally, we provide an analysis of between problem complexity and optimal module decomposition and evaluate the maintainability index, confirming that the code generated by MoTCoder is easier to understand and modify, which can be beneficial for long-term code maintenance and evolution. Our codes are available at https://github.com/dvlab-research/MoTCoder.

==> append_tables/apps_example_1.tex <==
\begin{table}[t]
    \centering
    \color{blue}
    \begin{tabular}{p{\linewidth}}
        \textbf{Original Solution} \\
\begin{lstlisting}
for _ in range(int(input())):
    s = input()

    ones = []
    cnt = 0
    for i in s:
        if i == '1':
            cnt += 1
        else:
            if cnt != 0:
                ones.append(cnt)
                cnt = 0
    if cnt != 0:
        ones.append(cnt)

    ones.sort(reverse=True)
    print(sum(ones[::2]))
\end{lstlisting} \\
        \textbf{MoT Solution} \\
\begin{lstlisting}
def calculate_alice_score(binary_string):
    """
    This function calculates Alice's score by extracting continuous segments of '1's, sorting them in descending order, and summing up the counts that Alice would pick.
    """
    ones_groups = []
    current_count = 0

    # Extract groups of consecutive '1's
    for char in binary_string:
        if char == '1':
            current_count += 1
        else:
            if current_count > 0:
                ones_groups.append(current_count)
                current_count = 0

    # Append the last segment if it ends with '1's
    if current_count > 0:
        ones_groups.append(current_count)

    # Sort segments in descending order to maximize Alice's score
    ones_groups.sort(reverse=True)

    # Alice selects the first, third, fifth ... largest groups
    return sum(ones_groups[::2])

# Process multiple test cases
test_cases = int(input())

for _ in range(test_cases):
    binary_string = input().strip()
    print(calculate_alice_score(binary_string))
\end{lstlisting} \\
    \end{tabular}
    \caption{Comparison of Original and MoT Solutions for Binary String Processing.}
    \label{tab:data_example}
\end{table}

==> append_tables/apps_problem_source.tex <==
\begin{table}[h]
\centering
\caption{The source of problems in APPS~\cite{hendrycksapps2021}. }
\small
\begin{tabular}{l|p{10cm}}
\toprule
Contest & Problems URL \\
\midrule
Codewars & \url{https://www.codewars.com/} \\ 
AtCoder & \url{https://atcoder.jp/} \\ 
Kattis & \url{https://open.kattis.com/} \\ 
Codeforces & \url{https://codeforces.com/} \\ 
\bottomrule
\end{tabular}
\label{tab:apps_problems}
\end{table}


==> append_tables/codecontests_problem_source.tex <==
\begin{table}[h]
\centering
% \setlength{\tabcolsep}{20mm}
\caption{The source of problems in CodeContests~\cite{li2022competition}. }
\small
\begin{tabular}{l|p{10cm}}
\toprule
Contest & Problems URL \\
\midrule
Aizu & \url{https://judge.u-aizu.ac.jp}  \\ 
AtCoder & \url{https://atcoder.jp}  \\
CodeChef & \url{https://www.codechef.com}  \\
Codeforces & \url{https://codeforces.com} \\
HackerEarth & \url{https://www.hackerearth.com} \\
\bottomrule
\end{tabular}
\label{tab:codecontests_problems}
\end{table}


==> append_tables/hyperparameters.tex <==
\begin{figure}[h]
    \centering
    \begin{minipage}{0.41\textwidth}
        \centering
        \setlength{\tabcolsep}{1mm}
        \captionof{table}{General Hyperparameters}
        \begin{tabular}{lc}
        \toprule
        Hyperparameter & Value \\
        \midrule
        num train epochs & 3 \\
        model max length & 2048 \\
        per device train batch size & 16 \\
        per device eval batch size & 1 \\
        gradient accumulation steps & 4 \\
        learning rate & $2 \times 10^{-5}$ \\
        warmup steps & 10 \\
        lr scheduler type & cosine \\
        gradient checkpointing & True \\
        bf16 & True \\
        \bottomrule
        \end{tabular}
        \label{tab:general_hyperparameters}
    \end{minipage}
    \hfill
    \begin{minipage}{0.57\textwidth}
        \centering
        \setlength{\tabcolsep}{0.8mm}
        \captionof{table}{Deepspeed-related Hyperparameters}
        \begin{tabular}{lc}
        \toprule
        Hyperparameter & Value \\
        \midrule
        optimizer & AdamW \\
        scheduler & WarmupLR \\
        zero optimization stage & 3 \\
        offload optimizer device & cpu \\
        offload optimizer pin memory & true \\
        offload param device & cpu \\
        offload param pin memory & true \\
        overlap comm & true \\
        contiguous gradients & true \\
        sub group size & $1 \times 10^{9}$ \\
        stage3 max live parameters & $1 \times 10^{9}$ \\
        stage3 max reuse distance & $1 \times 10^{9}$ \\
        stage3 gather 16bit weights on model save & true \\
        wall clock breakdown & false \\
        \bottomrule
        \end{tabular}
        \label{tab:deepspeed_hyperparameters}
    \end{minipage}
\end{figure}


==> append_tables/leetcode_problem_list.tex <==

% 
\small
\setlength{\tabcolsep}{1.5mm}
\begin{longtable}{cc|l}
\toprule
ID & Level & Problems URL \\
\midrule
\endfirsthead
\toprule
ID & Level & Problems URL \\
\midrule
\endhead
\bottomrule
\endfoot
\endlastfoot
1 & easy & \scriptsize \url{https://leetcode.com/problems/matrix-similarity-after-cyclic-shifts/} \\
2 & easy & \scriptsize \url{https://leetcode.com/problems/make-three-strings-equal/} \\
3 & easy & \scriptsize \url{https://leetcode.com/problems/distribute-candies-among-children-i/} \\
4 & easy & \scriptsize \url{https://leetcode.com/problems/find-words-containing-character/} \\
5 & easy & \scriptsize \url{https://leetcode.com/problems/maximum-strong-pair-xor-i/} \\
6 & easy & \scriptsize \url{https://leetcode.com/problems/find-champion-i/} \\
7 & easy & \scriptsize \url{https://leetcode.com/problems/find-the-k-or-of-an-array/} \\
8 & easy & \scriptsize \url{https://leetcode.com/problems/minimum-sum-of-mountain-triplets-i/} \\
9 & easy & \scriptsize \url{https://leetcode.com/problems/divisible-and-non-divisible-sums-difference/} \\
10 & easy & \scriptsize \url{https://leetcode.com/problems/find-indices-with-index-and-value-difference-i/} \\
11 & easy & \scriptsize \url{https://leetcode.com/problems/last-visited-integers/} \\
12 & easy & \scriptsize \url{https://leetcode.com/problems/subarrays-distinct-element-sum-of-squares-i/} \\
13 & easy & \scriptsize \url{https://leetcode.com/problems/maximum-value-of-an-ordered-triplet-i/} \\
14 & easy & \scriptsize \url{https://leetcode.com/problems/sum-of-values-at-indices-with-k-set-bits/} \\
15 & easy & \scriptsize \url{https://leetcode.com/problems/maximum-odd-binary-number/} \\
16 & easy & \scriptsize \url{https://leetcode.com/problems/minimum-right-shifts-to-sort-the-array/} \\
17 & easy & \scriptsize \url{https://leetcode.com/problems/minimum-operations-to-collect-elements/} \\
18 & easy & \scriptsize \url{https://leetcode.com/problems/points-that-intersect-with-cars/} \\
19 & easy & \scriptsize \url{https://leetcode.com/problems/furthest-point-from-origin/} \\
20 & easy & \scriptsize \url{https://leetcode.com/problems/check-if-strings-can-be-made-equal-with-operations-i/} \\
21 & easy & \scriptsize \url{https://leetcode.com/problems/count-symmetric-integers/} \\
22 & easy & \scriptsize \url{https://leetcode.com/problems/check-if-a-string-is-an-acronym-of-words/} \\
23 & easy & \scriptsize \url{https://leetcode.com/problems/account-balance-after-rounded-purchase/} \\
24 & easy & \scriptsize \url{https://leetcode.com/problems/count-pairs-whose-sum-is-less-than-target/} \\
25 & easy & \scriptsize \url{https://leetcode.com/problems/max-pair-sum-in-an-array/} \\
26 & easy & \scriptsize \url{https://leetcode.com/problems/check-if-array-is-good/} \\
27 & easy & \scriptsize \url{https://leetcode.com/problems/faulty-keyboard/} \\
28 & easy & \scriptsize \url{https://leetcode.com/problems/split-strings-by-separator/} \\
29 & easy & \scriptsize \url{https://leetcode.com/problems/number-of-employees-who-met-the-target/} \\
30 & easy & \scriptsize \url{https://leetcode.com/problems/longest-alternating-subarray/} \\
31 & easy & \scriptsize \url{https://leetcode.com/problems/longest-even-odd-subarray-with-threshold/} \\
32 & easy & \scriptsize \url{https://leetcode.com/problems/total-distance-traveled/} \\
33 & easy & \scriptsize \url{https://leetcode.com/problems/find-maximum-number-of-string-pairs/} \\
34 & easy & \scriptsize \url{https://leetcode.com/problems/sum-of-squares-of-special-elements/} \\
35 & easy & \scriptsize \url{https://leetcode.com/problems/neither-minimum-nor-maximum/} \\
36 & easy & \scriptsize \url{https://leetcode.com/problems/number-of-beautiful-pairs/} \\
37 & easy & \scriptsize \url{https://leetcode.com/problems/minimize-string-length/} \\
38 & easy & \scriptsize \url{https://leetcode.com/problems/check-if-the-number-is-fascinating/} \\
39 & easy & \scriptsize \url{https://leetcode.com/problems/remove-trailing-zeros-from-a-string/} \\
40 & easy & \scriptsize \url{https://leetcode.com/problems/lexicographically-smallest-palindrome/} \\
41 & easy & \scriptsize \url{https://leetcode.com/problems/find-the-maximum-achievable-number/} \\
42 & easy & \scriptsize \url{https://leetcode.com/problems/minimum-string-length-after-removing-substrings/} \\
43 & easy & \scriptsize \url{https://leetcode.com/problems/find-the-losers-of-the-circular-game/} \\
44 & easy & \scriptsize \url{https://leetcode.com/problems/semi-ordered-permutation/} \\
45 & easy & \scriptsize \url{https://leetcode.com/problems/find-the-distinct-difference-array/} \\
46 & easy & \scriptsize \url{https://leetcode.com/problems/maximum-sum-with-exactly-k-elements/} \\
47 & easy & \scriptsize \url{https://leetcode.com/problems/buy-two-chocolates/} \\
48 & easy & \scriptsize \url{https://leetcode.com/problems/sum-multiples/} \\
49 & easy & \scriptsize \url{https://leetcode.com/problems/calculate-delayed-arrival-time/} \\
50 & easy & \scriptsize \url{https://leetcode.com/problems/row-with-maximum-ones/} \\
51 & easy & \scriptsize \url{https://leetcode.com/problems/number-of-senior-citizens/} \\
52 & easy & \scriptsize \url{https://leetcode.com/problems/find-the-longest-balanced-substring-of-a-binary-string/} \\
53 & easy & \scriptsize \url{https://leetcode.com/problems/prime-in-diagonal/} \\
54 & easy & \scriptsize \url{https://leetcode.com/problems/k-items-with-the-maximum-sum/} \\
55 & easy & \scriptsize \url{https://leetcode.com/problems/left-and-right-sum-differences/} \\
56 & easy & \scriptsize \url{https://leetcode.com/problems/merge-two-2d-arrays-by-summing-values/} \\
57 & easy & \scriptsize \url{https://leetcode.com/problems/maximum-difference-by-remapping-a-digit/} \\
58 & easy & \scriptsize \url{https://leetcode.com/problems/find-the-array-concatenation-value/} \\
59 & easy & \scriptsize \url{https://leetcode.com/problems/find-the-maximum-divisibility-score/} \\
60 & easy & \scriptsize \url{https://leetcode.com/problems/take-gifts-from-the-richest-pile/} \\
61 & easy & \scriptsize \url{https://leetcode.com/problems/determine-the-winner-of-a-bowling-game/} \\
62 & easy & \scriptsize \url{https://leetcode.com/problems/count-distinct-numbers-on-board/} \\
63 & easy & \scriptsize \url{https://leetcode.com/problems/find-the-width-of-columns-of-a-grid/} \\
64 & easy & \scriptsize \url{https://leetcode.com/problems/form-smallest-number-from-two-digit-arrays/} \\
65 & easy & \scriptsize \url{https://leetcode.com/problems/distribute-money-to-maximum-children/} \\
66 & easy & \scriptsize \url{https://leetcode.com/problems/number-of-even-and-odd-bits/} \\
67 & easy & \scriptsize \url{https://leetcode.com/problems/count-the-number-of-vowel-strings-in-range/} \\
68 & easy & \scriptsize \url{https://leetcode.com/problems/split-with-minimum-sum/} \\
69 & easy & \scriptsize \url{https://leetcode.com/problems/pass-the-pillow/} \\
70 & easy & \scriptsize \url{https://leetcode.com/problems/separate-the-digits-in-an-array/} \\
71 & easy & \scriptsize \url{https://leetcode.com/problems/minimum-common-value/} \\
72 & easy & \scriptsize \url{https://leetcode.com/problems/alternating-digit-sum/} \\
73 & easy & \scriptsize \url{https://leetcode.com/problems/difference-between-element-sum-and-digit-sum-of-an-array/} \\
74 & easy & \scriptsize \url{https://leetcode.com/problems/categorize-box-according-to-criteria/} \\
75 & easy & \scriptsize \url{https://leetcode.com/problems/maximum-count-of-positive-integer-and-negative-integer/} \\
76 & easy & \scriptsize \url{https://leetcode.com/problems/count-the-digits-that-divide-a-number/} \\
77 & easy & \scriptsize \url{https://leetcode.com/problems/maximum-enemy-forts-that-can-be-captured/} \\
78 & easy & \scriptsize \url{https://leetcode.com/problems/shortest-distance-to-target-string-in-a-circular-array/} \\
79 & easy & \scriptsize \url{https://leetcode.com/problems/count-pairs-of-similar-strings/} \\
80 & easy & \scriptsize \url{https://leetcode.com/problems/maximum-value-of-a-string-in-an-array/} \\
81 & easy & \scriptsize \url{https://leetcode.com/problems/delete-greatest-value-in-each-row/} \\
82 & easy & \scriptsize \url{https://leetcode.com/problems/circular-sentence/} \\
83 & easy & \scriptsize \url{https://leetcode.com/problems/minimum-cuts-to-divide-a-circle/} \\
84 & easy & \scriptsize \url{https://leetcode.com/problems/find-the-pivot-integer/} \\
85 & easy & \scriptsize \url{https://leetcode.com/problems/number-of-unequal-triplets-in-array/} \\
86 & easy & \scriptsize \url{https://leetcode.com/problems/number-of-distinct-averages/} \\
87 & easy & \scriptsize \url{https://leetcode.com/problems/convert-the-temperature/} \\
88 & easy & \scriptsize \url{https://leetcode.com/problems/apply-operations-to-an-array/} \\
89 & easy & \scriptsize \url{https://leetcode.com/problems/odd-string-difference/} \\
90 & easy & \scriptsize \url{https://leetcode.com/problems/average-value-of-even-numbers-that-are-divisible-by-three/} \\
91 & easy & \scriptsize \url{https://leetcode.com/problems/determine-if-two-events-have-conflict/} \\
92 & easy & \scriptsize \url{https://leetcode.com/problems/remove-letter-to-equalize-frequency/} \\
93 & easy & \scriptsize \url{https://leetcode.com/problems/number-of-valid-clock-times/} \\
94 & hard & \scriptsize \url{https://leetcode.com/problems/find-maximum-non-decreasing-array-length/} \\
95 & hard & \scriptsize \url{https://leetcode.com/problems/count-beautiful-substrings-ii/} \\
96 & hard & \scriptsize \url{https://leetcode.com/problems/maximum-strong-pair-xor-ii/} \\
97 & hard & \scriptsize \url{https://leetcode.com/problems/maximum-balanced-subsequence-sum/} \\
98 & hard & \scriptsize \url{https://leetcode.com/problems/find-building-where-alice-and-bob-can-meet/} \\
99 & hard & \scriptsize \url{https://leetcode.com/problems/maximum-points-after-collecting-coins-from-all-nodes/} \\
100 & hard & \scriptsize \url{https://leetcode.com/problems/apply-operations-on-array-to-maximize-sum-of-squares/} \\
101 & hard & \scriptsize \url{https://leetcode.com/problems/count-visited-nodes-in-a-directed-graph/} \\
102 & hard & \scriptsize \url{https://leetcode.com/problems/subarrays-distinct-element-sum-of-squares-ii/} \\
103 & hard & \scriptsize \url{https://leetcode.com/problems/count-valid-paths-in-a-tree/} \\
104 & hard & \scriptsize \url{https://leetcode.com/problems/maximum-spending-after-buying-items/} \\
105 & hard & \scriptsize \url{https://leetcode.com/problems/minimum-edge-reversals-so-every-node-is-reachable/} \\
106 & hard & \scriptsize \url{https://leetcode.com/problems/count-of-sub-multisets-with-bounded-sum/} \\
107 & hard & \scriptsize \url{https://leetcode.com/problems/minimum-edge-weight-equilibrium-queries-in-a-tree/} \\
108 & hard & \scriptsize \url{https://leetcode.com/problems/maximum-number-of-k-divisible-components/} \\
109 & hard & \scriptsize \url{https://leetcode.com/problems/count-k-subsequences-of-a-string-with-maximum-beauty/} \\
110 & hard & \scriptsize \url{https://leetcode.com/problems/maximum-element-sum-of-a-complete-subset-of-indices/} \\
111 & hard & \scriptsize \url{https://leetcode.com/problems/maximize-value-of-function-in-a-ball-passing-game/} \\
112 & hard & \scriptsize \url{https://leetcode.com/problems/minimum-operations-to-form-subsequence-with-target-sum/} \\
113 & hard & \scriptsize \url{https://leetcode.com/problems/string-transformation/} \\
114 & hard & \scriptsize \url{https://leetcode.com/problems/number-of-beautiful-integers-in-the-range/} \\
115 & hard & \scriptsize \url{https://leetcode.com/problems/apply-operations-to-maximize-score/} \\
116 & hard & \scriptsize \url{https://leetcode.com/problems/minimum-time-to-make-array-sum-at-most-x/} \\
117 & hard & \scriptsize \url{https://leetcode.com/problems/count-stepping-numbers-in-range/} \\
118 & hard & \scriptsize \url{https://leetcode.com/problems/maximum-number-of-groups-with-increasing-length/} \\
119 & hard & \scriptsize \url{https://leetcode.com/problems/count-paths-that-can-form-a-palindrome-in-a-tree/} \\
120 & hard & \scriptsize \url{https://leetcode.com/problems/maximum-elegance-of-a-k-length-subsequence/} \\
121 & hard & \scriptsize \url{https://leetcode.com/problems/length-of-the-longest-valid-substring/} \\
122 & hard & \scriptsize \url{https://leetcode.com/problems/minimum-changes-to-make-k-semi-palindromes/} \\
123 & hard & \scriptsize \url{https://leetcode.com/problems/sum-of-imbalance-numbers-of-all-subarrays/} \\
124 & hard & \scriptsize \url{https://leetcode.com/problems/robot-collisions/} \\
125 & hard & \scriptsize \url{https://leetcode.com/problems/maximum-sum-queries/} \\
126 & hard & \scriptsize \url{https://leetcode.com/problems/greatest-common-divisor-traversal/} \\
127 & hard & \scriptsize \url{https://leetcode.com/problems/find-a-good-subset-of-the-matrix/} \\
128 & hard & \scriptsize \url{https://leetcode.com/problems/maximum-strictly-increasing-cells-in-a-matrix/} \\
129 & hard & \scriptsize \url{https://leetcode.com/problems/painting-the-walls/} \\
130 & hard & \scriptsize \url{https://leetcode.com/problems/modify-graph-edge-weights/} \\
131 & hard & \scriptsize \url{https://leetcode.com/problems/power-of-heroes/} \\
132 & hard & \scriptsize \url{https://leetcode.com/problems/make-array-empty/} \\
133 & hard & \scriptsize \url{https://leetcode.com/problems/count-of-integers/} \\
134 & hard & \scriptsize \url{https://leetcode.com/problems/minimize-the-total-price-of-the-trips/} \\
135 & hard & \scriptsize \url{https://leetcode.com/problems/minimum-reverse-operations/} \\
136 & hard & \scriptsize \url{https://leetcode.com/problems/collect-coins-in-a-tree/} \\
137 & hard & \scriptsize \url{https://leetcode.com/problems/minimum-time-to-visit-a-cell-in-a-grid/} \\
138 & hard & \scriptsize \url{https://leetcode.com/problems/find-the-string-with-lcp/} \\
139 & hard & \scriptsize \url{https://leetcode.com/problems/handling-sum-queries-after-update/} \\
140 & hard & \scriptsize \url{https://leetcode.com/problems/subsequence-with-the-minimum-score/} \\
141 & hard & \scriptsize \url{https://leetcode.com/problems/minimum-number-of-visited-cells-in-a-grid/} \\
142 & hard & \scriptsize \url{https://leetcode.com/problems/rearranging-fruits/} \\
143 & hard & \scriptsize \url{https://leetcode.com/problems/lexicographically-smallest-beautiful-string/} \\
144 & hard & \scriptsize \url{https://leetcode.com/problems/count-increasing-quadruplets/} \\
145 & hard & \scriptsize \url{https://leetcode.com/problems/put-marbles-in-bags/} \\
146 & hard & \scriptsize \url{https://leetcode.com/problems/shortest-cycle-in-a-graph/} \\
147 & hard & \scriptsize \url{https://leetcode.com/problems/minimum-time-to-complete-all-tasks/} \\
148 & hard & \scriptsize \url{https://leetcode.com/problems/count-number-of-possible-root-nodes/} \\
149 & hard & \scriptsize \url{https://leetcode.com/problems/number-of-ways-to-earn-points/} \\
150 & hard & \scriptsize \url{https://leetcode.com/problems/split-the-array-to-make-coprime-products/} \\
151 & hard & \scriptsize \url{https://leetcode.com/problems/time-to-cross-a-bridge/} \\
152 & hard & \scriptsize \url{https://leetcode.com/problems/check-if-point-is-reachable/} \\
153 & hard & \scriptsize \url{https://leetcode.com/problems/minimum-cost-to-split-an-array/} \\
154 & hard & \scriptsize \url{https://leetcode.com/problems/difference-between-maximum-and-minimum-price-sum/} \\
155 & hard & \scriptsize \url{https://leetcode.com/problems/maximize-the-minimum-powered-city/} \\
156 & hard & \scriptsize \url{https://leetcode.com/problems/count-anagrams/} \\
157 & hard & \scriptsize \url{https://leetcode.com/problems/number-of-great-partitions/} \\
158 & hard & \scriptsize \url{https://leetcode.com/problems/cycle-length-queries-in-a-tree/} \\
159 & hard & \scriptsize \url{https://leetcode.com/problems/add-edges-to-make-degrees-of-all-nodes-even/} \\
160 & hard & \scriptsize \url{https://leetcode.com/problems/minimum-total-cost-to-make-arrays-unequal/} \\
161 & hard & \scriptsize \url{https://leetcode.com/problems/maximum-number-of-points-from-grid-queries/} \\
162 & hard & \scriptsize \url{https://leetcode.com/problems/divide-nodes-into-the-maximum-number-of-groups/} \\
163 & hard & \scriptsize \url{https://leetcode.com/problems/count-palindromic-subsequences/} \\
164 & hard & \scriptsize \url{https://leetcode.com/problems/count-subarrays-with-median-k/} \\
165 & hard & \scriptsize \url{https://leetcode.com/problems/number-of-beautiful-partitions/} \\
166 & hard & \scriptsize \url{https://leetcode.com/problems/split-message-based-on-limit/} \\
167 & hard & \scriptsize \url{https://leetcode.com/problems/maximum-number-of-non-overlapping-palindrome-substrings/} \\
168 & hard & \scriptsize \url{https://leetcode.com/problems/minimum-total-distance-traveled/} \\
169 & hard & \scriptsize \url{https://leetcode.com/problems/next-greater-element-iv/} \\
170 & hard & \scriptsize \url{https://leetcode.com/problems/minimum-number-of-operations-to-make-arrays-similar/} \\
171 & hard & \scriptsize \url{https://leetcode.com/problems/minimum-cost-to-make-array-equal/} \\
172 & hard & \scriptsize \url{https://leetcode.com/problems/create-components-with-same-value/} \\
173 & hard & \scriptsize \url{https://leetcode.com/problems/count-subarrays-with-fixed-bounds/} \\
174 & hard & \scriptsize \url{https://leetcode.com/problems/longest-increasing-subsequence-ii/} \\
175 & hard & \scriptsize \url{https://leetcode.com/problems/paths-in-matrix-whose-sum-is-divisible-by-k/} \\
176 & medium & \scriptsize \url{https://leetcode.com/problems/make-lexicographically-smallest-array-by-swapping-elements/} \\
177 & medium & \scriptsize \url{https://leetcode.com/problems/maximize-area-of-square-hole-in-grid/} \\
178 & medium & \scriptsize \url{https://leetcode.com/problems/count-beautiful-substrings-i/} \\
179 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-number-of-coins-for-fruits/} \\
180 & medium & \scriptsize \url{https://leetcode.com/problems/high-access-employees/} \\
181 & medium & \scriptsize \url{https://leetcode.com/problems/distribute-candies-among-children-ii/} \\
182 & medium & \scriptsize \url{https://leetcode.com/problems/number-of-strings-which-can-be-rearranged-to-contain-substring/} \\
183 & medium & \scriptsize \url{https://leetcode.com/problems/separate-black-and-white-balls/} \\
184 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-xor-product/} \\
185 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-score-after-applying-operations-on-a-tree/} \\
186 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-operations-to-maximize-last-elements-in-arrays/} \\
187 & medium & \scriptsize \url{https://leetcode.com/problems/find-champion-ii/} \\
188 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-sum-of-mountain-triplets-ii/} \\
189 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-increment-operations-to-make-array-beautiful/} \\
190 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-number-of-changes-to-make-binary-string-beautiful/} \\
191 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-equal-sum-of-two-arrays-after-replacing-zeros/} \\
192 & medium & \scriptsize \url{https://leetcode.com/problems/find-indices-with-index-and-value-difference-ii/} \\
193 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-number-of-groups-to-create-a-valid-assignment/} \\
194 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-value-of-an-ordered-triplet-ii/} \\
195 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-processing-time/} \\
196 & medium & \scriptsize \url{https://leetcode.com/problems/shortest-and-lexicographically-smallest-beautiful-string/} \\
197 & medium & \scriptsize \url{https://leetcode.com/problems/longest-unequal-adjacent-groups-subsequence-i/} \\
198 & medium & \scriptsize \url{https://leetcode.com/problems/longest-unequal-adjacent-groups-subsequence-ii/} \\
199 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-size-subarray-in-infinite-array/} \\
200 & medium & \scriptsize \url{https://leetcode.com/problems/beautiful-towers-i/} \\
201 & medium & \scriptsize \url{https://leetcode.com/problems/beautiful-towers-ii/} \\
202 & medium & \scriptsize \url{https://leetcode.com/problems/length-of-the-longest-subsequence-that-sums-to-target/} \\
203 & medium & \scriptsize \url{https://leetcode.com/problems/happy-students/} \\
204 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-number-of-alloys/} \\
205 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-number-of-operations-to-make-array-empty/} \\
206 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-moves-to-spread-stones-over-grid/} \\
207 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-array-length-after-pair-removals/} \\
208 & medium & \scriptsize \url{https://leetcode.com/problems/split-array-into-maximum-number-of-subarrays/} \\
209 & medium & \scriptsize \url{https://leetcode.com/problems/determine-if-a-cell-is-reachable-at-a-given-time/} \\
210 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-operations-to-make-a-special-number/} \\
211 & medium & \scriptsize \url{https://leetcode.com/problems/apply-operations-to-make-two-strings-equal/} \\
212 & medium & \scriptsize \url{https://leetcode.com/problems/construct-product-matrix/} \\
213 & medium & \scriptsize \url{https://leetcode.com/problems/find-the-minimum-possible-sum-of-a-beautiful-array/} \\
214 & medium & \scriptsize \url{https://leetcode.com/problems/make-string-a-subsequence-using-cyclic-increments/} \\
215 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-absolute-difference-between-elements-with-constraint/} \\
216 & medium & \scriptsize \url{https://leetcode.com/problems/maximize-the-profit-as-the-salesman/} \\
217 & medium & \scriptsize \url{https://leetcode.com/problems/check-if-strings-can-be-made-equal-with-operations-ii/} \\
218 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-sum-of-almost-unique-subarray/} \\
219 & medium & \scriptsize \url{https://leetcode.com/problems/count-pairs-of-points-with-distance-k/} \\
220 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-seconds-to-equalize-a-circular-array/} \\
221 & medium & \scriptsize \url{https://leetcode.com/problems/check-if-it-is-possible-to-split-array/} \\
222 & medium & \scriptsize \url{https://leetcode.com/problems/count-of-interesting-subarrays/} \\
223 & medium & \scriptsize \url{https://leetcode.com/problems/find-the-safest-path-in-a-grid/} \\
224 & medium & \scriptsize \url{https://leetcode.com/problems/sorting-three-groups/} \\
225 & medium & \scriptsize \url{https://leetcode.com/problems/visit-array-positions-to-maximize-score/} \\
226 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-beauty-of-an-array-after-applying-operation/} \\
227 & medium & \scriptsize \url{https://leetcode.com/problems/number-of-black-blocks/} \\
228 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-index-of-a-valid-split/} \\
229 & medium & \scriptsize \url{https://leetcode.com/problems/sort-vowels-in-a-string/} \\
230 & medium & \scriptsize \url{https://leetcode.com/problems/partition-string-into-minimum-beautiful-substrings/} \\
231 & medium & \scriptsize \url{https://leetcode.com/problems/ways-to-express-an-integer-as-sum-of-powers/} \\
232 & medium & \scriptsize \url{https://leetcode.com/problems/apply-operations-to-make-all-array-elements-equal-to-zero/} \\
233 & medium & \scriptsize \url{https://leetcode.com/problems/shortest-string-that-contains-three-strings/} \\
234 & medium & \scriptsize \url{https://leetcode.com/problems/prime-pairs-with-target-sum/} \\
235 & medium & \scriptsize \url{https://leetcode.com/problems/largest-element-in-an-array-after-merge-operations/} \\
236 & medium & \scriptsize \url{https://leetcode.com/problems/longest-non-decreasing-subarray-from-two-arrays/} \\
237 & medium & \scriptsize \url{https://leetcode.com/problems/continuous-subarrays/} \\
238 & medium & \scriptsize \url{https://leetcode.com/problems/ways-to-split-array-into-good-subarrays/} \\
239 & medium & \scriptsize \url{https://leetcode.com/problems/count-complete-subarrays-in-an-array/} \\
240 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-number-of-jumps-to-reach-the-last-index/} \\
241 & medium & \scriptsize \url{https://leetcode.com/problems/decremental-string-concatenation/} \\
242 & medium & \scriptsize \url{https://leetcode.com/problems/construct-the-longest-new-string/} \\
243 & medium & \scriptsize \url{https://leetcode.com/problems/special-permutations/} \\
244 & medium & \scriptsize \url{https://leetcode.com/problems/find-the-value-of-the-partition/} \\
245 & medium & \scriptsize \url{https://leetcode.com/problems/sum-of-matrix-after-queries/} \\
246 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-operations-to-make-the-integer-zero/} \\
247 & medium & \scriptsize \url{https://leetcode.com/problems/relocate-marbles/} \\
248 & medium & \scriptsize \url{https://leetcode.com/problems/count-zero-request-servers/} \\
249 & medium & \scriptsize \url{https://leetcode.com/problems/find-the-longest-equal-subarray/} \\
250 & medium & \scriptsize \url{https://leetcode.com/problems/lexicographically-smallest-string-after-substring-operation/} \\
251 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-cost-to-make-all-characters-equal/} \\
252 & medium & \scriptsize \url{https://leetcode.com/problems/determine-the-minimum-sum-of-a-k-avoiding-array/} \\
253 & medium & \scriptsize \url{https://leetcode.com/problems/collecting-chocolates/} \\
254 & medium & \scriptsize \url{https://leetcode.com/problems/find-the-punishment-number-of-an-integer/} \\
255 & medium & \scriptsize \url{https://leetcode.com/problems/difference-of-number-of-distinct-values-on-diagonals/} \\
256 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-number-of-moves-in-a-grid/} \\
257 & medium & \scriptsize \url{https://leetcode.com/problems/count-the-number-of-complete-components/} \\
258 & medium & \scriptsize \url{https://leetcode.com/problems/neighboring-bitwise-xor/} \\
259 & medium & \scriptsize \url{https://leetcode.com/problems/movement-of-robots/} \\
260 & medium & \scriptsize \url{https://leetcode.com/problems/find-the-longest-semi-repetitive-substring/} \\
261 & medium & \scriptsize \url{https://leetcode.com/problems/make-costs-of-paths-equal-in-a-binary-tree/} \\
262 & medium & \scriptsize \url{https://leetcode.com/problems/number-of-adjacent-elements-with-the-same-color/} \\
263 & medium & \scriptsize \url{https://leetcode.com/problems/find-the-prefix-common-array-of-two-arrays/} \\
264 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-number-of-fish-in-a-grid/} \\
265 & medium & \scriptsize \url{https://leetcode.com/problems/extra-characters-in-a-string/} \\
266 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-strength-of-a-group/} \\
267 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-number-of-operations-to-make-all-array-elements-equal-to-1/} \\
268 & medium & \scriptsize \url{https://leetcode.com/problems/sliding-subarray-beauty/} \\
269 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-additions-to-make-valid-string/} \\
270 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-or/} \\
271 & medium & \scriptsize \url{https://leetcode.com/problems/sum-in-a-matrix/} \\
272 & medium & \scriptsize \url{https://leetcode.com/problems/mice-and-cheese/} \\
273 & medium & \scriptsize \url{https://leetcode.com/problems/convert-an-array-into-a-2d-array-with-conditions/} \\
274 & medium & \scriptsize \url{https://leetcode.com/problems/sum-of-distances/} \\
275 & medium & \scriptsize \url{https://leetcode.com/problems/minimize-the-maximum-difference-of-pairs/} \\
276 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-operations-to-make-all-array-elements-equal/} \\
277 & medium & \scriptsize \url{https://leetcode.com/problems/prime-subtraction-operation/} \\
278 & medium & \scriptsize \url{https://leetcode.com/problems/find-the-divisibility-array-of-a-string/} \\
279 & medium & \scriptsize \url{https://leetcode.com/problems/find-the-maximum-number-of-marked-indices/} \\
280 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-operations-to-reduce-an-integer-to-0/} \\
281 & medium & \scriptsize \url{https://leetcode.com/problems/count-the-number-of-square-free-subsets/} \\
282 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-score-by-changing-two-elements/} \\
283 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-impossible-or/} \\
284 & medium & \scriptsize \url{https://leetcode.com/problems/substring-xor-queries/} \\
285 & medium & \scriptsize \url{https://leetcode.com/problems/count-the-number-of-fair-pairs/} \\
286 & medium & \scriptsize \url{https://leetcode.com/problems/the-number-of-beautiful-subsets/} \\
287 & medium & \scriptsize \url{https://leetcode.com/problems/find-score-of-an-array-after-marking-all-elements/} \\
288 & medium & \scriptsize \url{https://leetcode.com/problems/count-vowel-strings-in-ranges/} \\
289 & medium & \scriptsize \url{https://leetcode.com/problems/house-robber-iv/} \\
290 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-cost-of-a-path-with-special-roads/} \\
291 & medium & \scriptsize \url{https://leetcode.com/problems/first-completely-painted-row-or-column/} \\
292 & medium & \scriptsize \url{https://leetcode.com/problems/count-collisions-of-monkeys-on-a-polygon/} \\
293 & medium & \scriptsize \url{https://leetcode.com/problems/find-the-score-of-all-prefixes-of-an-array/} \\
294 & medium & \scriptsize \url{https://leetcode.com/problems/maximize-win-from-two-segments/} \\
295 & medium & \scriptsize \url{https://leetcode.com/problems/make-k-subarray-sums-equal/} \\
296 & medium & \scriptsize \url{https://leetcode.com/problems/find-the-substring-with-maximum-cost/} \\
297 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-time-to-repair-cars/} \\
298 & medium & \scriptsize \url{https://leetcode.com/problems/maximize-greatness-of-an-array/} \\
299 & medium & \scriptsize \url{https://leetcode.com/problems/check-knight-tour-configuration/} \\
300 & medium & \scriptsize \url{https://leetcode.com/problems/smallest-missing-non-negative-integer-after-operations/} \\
301 & medium & \scriptsize \url{https://leetcode.com/problems/count-the-number-of-beautiful-subarrays/} \\
302 & medium & \scriptsize \url{https://leetcode.com/problems/rearrange-array-to-maximize-prefix-score/} \\
303 & medium & \scriptsize \url{https://leetcode.com/problems/count-ways-to-group-overlapping-ranges/} \\
304 & medium & \scriptsize \url{https://leetcode.com/problems/count-total-number-of-colored-cells/} \\
305 & medium & \scriptsize \url{https://leetcode.com/problems/disconnect-path-in-a-binary-matrix-by-at-most-one-flip/} \\
306 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-number-of-integers-to-choose-from-a-range-i/} \\
307 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-subsequence-score/} \\
308 & medium & \scriptsize \url{https://leetcode.com/problems/apply-bitwise-operations-to-make-strings-equal/} \\
309 & medium & \scriptsize \url{https://leetcode.com/problems/sort-the-students-by-their-kth-score/} \\
310 & medium & \scriptsize \url{https://leetcode.com/problems/minimize-the-maximum-of-two-arrays/} \\
311 & medium & \scriptsize \url{https://leetcode.com/problems/count-the-number-of-good-subarrays/} \\
312 & medium & \scriptsize \url{https://leetcode.com/problems/increment-submatrices-by-one/} \\
313 & medium & \scriptsize \url{https://leetcode.com/problems/find-xor-beauty-of-array/} \\
314 & medium & \scriptsize \url{https://leetcode.com/problems/maximal-score-after-applying-k-operations/} \\
315 & medium & \scriptsize \url{https://leetcode.com/problems/make-number-of-distinct-characters-equal/} \\
316 & medium & \scriptsize \url{https://leetcode.com/problems/closest-prime-numbers-in-range/} \\
317 & medium & \scriptsize \url{https://leetcode.com/problems/distinct-prime-factors-of-product-of-array/} \\
318 & medium & \scriptsize \url{https://leetcode.com/problems/difference-between-ones-and-zeros-in-row-and-column/} \\
319 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-operations-to-make-array-equal-ii/} \\
320 & medium & \scriptsize \url{https://leetcode.com/problems/reward-top-k-students/} \\
321 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-tastiness-of-candy-basket/} \\
322 & medium & \scriptsize \url{https://leetcode.com/problems/take-k-of-each-character-from-left-and-right/} \\
323 & medium & \scriptsize \url{https://leetcode.com/problems/smallest-value-after-replacing-with-sum-of-prime-factors/} \\
324 & medium & \scriptsize \url{https://leetcode.com/problems/frog-jump-ii/} \\
325 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-star-sum-of-a-graph/} \\
326 & medium & \scriptsize \url{https://leetcode.com/problems/longest-square-streak-in-an-array/} \\
327 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-score-of-a-path-between-two-cities/} \\
328 & medium & \scriptsize \url{https://leetcode.com/problems/divide-players-into-teams-of-equal-skill/} \\
329 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-penalty-for-a-shop/} \\
330 & medium & \scriptsize \url{https://leetcode.com/problems/append-characters-to-string-to-make-subsequence/} \\
331 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-fuel-cost-to-report-to-the-capital/} \\
332 & medium & \scriptsize \url{https://leetcode.com/problems/most-profitable-path-in-a-tree/} \\
333 & medium & \scriptsize \url{https://leetcode.com/problems/count-ways-to-build-good-strings/} \\
334 & medium & \scriptsize \url{https://leetcode.com/problems/number-of-subarrays-with-lcm-equal-to-k/} \\
335 & medium & \scriptsize \url{https://leetcode.com/problems/total-cost-to-hire-k-workers/} \\
336 & medium & \scriptsize \url{https://leetcode.com/problems/maximum-sum-of-distinct-subarrays-with-length-k/} \\
337 & medium & \scriptsize \url{https://leetcode.com/problems/words-within-two-edits-of-dictionary/} \\
338 & medium & \scriptsize \url{https://leetcode.com/problems/destroy-sequential-targets/} \\
339 & medium & \scriptsize \url{https://leetcode.com/problems/number-of-subarrays-with-gcd-equal-to-k/} \\
340 & medium & \scriptsize \url{https://leetcode.com/problems/minimum-addition-to-make-integer-beautiful/} \\
341 & medium & \scriptsize \url{https://leetcode.com/problems/most-popular-video-creator/} \\
342 & medium & \scriptsize \url{https://leetcode.com/problems/sum-of-number-and-its-reverse/} \\
343 & medium & \scriptsize \url{https://leetcode.com/problems/bitwise-xor-of-all-pairings/} \\
344 & medium & \scriptsize \url{https://leetcode.com/problems/minimize-maximum-of-array/} \\
345 & medium & \scriptsize \url{https://leetcode.com/problems/range-product-queries-of-powers/} \\
\bottomrule
\caption{\normalsize LeetCode problem list.}
\label{tab:leetcode_problem_list}\\
\end{longtable}
\normalsize

==> tables/ablation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% CoT ablation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{table*}[t]
\centering
\caption{\textbf{Modular-of-thought instruction tuning ablation experiments}. We compare the one-step and two-step modular-of-thought instruction tuning strategies. Models are inferred using both normal and modular prompts. APPs test results by \emph{pass@1} (\%) are shown.}

% \setlength{\tabcolsep}{3.6mm}
\setlength{\tabcolsep}{5.9mm}
\begin{tabular}{lcc|cccc}
\toprule
Model & Size & Prompt & Introductory & Interview & Competition & All \\
\midrule
% results train on the single dataset
 & & Normal  & 30.76 & 17.16 & 11.16 & 18.68 \\
\multirow{-2}{*}{1-Step MoTCoder} & \multirow{-2}{*}{15B} & Modular & 31.69 & 17.37 & 11.47 & 19.05 \\
\midrule 
% results train on the single dataset
% \rowcolor{gray!20} & & Normal & 31.96 & 17.72 & 12.49 & 19.52 \\
% \rowcolor{gray!20} \multirow{-2}{*}{2-Step MoTCoder} & \multirow{-2}{*}{15B} & CoT & 32.51 & 18.45 &11.38 & 19.84\\
\rowcolor{gray!20} & & Normal & \appsinter{} & \appsintro{} & \appscom{} & \appsavg{} \\
\rowcolor{gray!20} \multirow{-2}{*}{2-Step MoTCoder} & \multirow{-2}{*}{15B} & Modular & 35.86 & 18.79 & 11.82 & 20.81 \\
\bottomrule
\end{tabular}
\label{tab:cot}
\end{table*}
\fi

%%%%%% Lora
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{table*}[t]
\centering
\caption{\textbf{Lora Training}. We compare the fully and Lora MoT instruction finetuning strategies. APPs test results by \emph{pass@1} (\%) are shown.}

\setlength{\tabcolsep}{6mm}
\begin{tabular}{lc|cccc}
\toprule
Model & Parameters & Introductory & Interview & Competition & All \\
\midrule
% Lora Finetuning & & 33.80 & 19.70 & 11.09 & 20.80 \\
\rowcolor{gray!20} Fully Finetuning & & 33.86 & 18.95 & 10.18 & 20.18 \\
\bottomrule
\end{tabular}
\label{tab:lora}
\end{table*}
\fi 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Datasets Ablation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\centering
\normalsize
\caption{Ablation experiment on training datasets. We compare MoTCoder training on normal and modular-of-thought dataset. APPs test results by \emph{pass@1} (\%) are shown.}
 \setlength{\tabcolsep}{3mm}
\begin{tabular}{lr|cccc}
\toprule
Model & Size & Introductory & Interview & Competition & All \\
\midrule
Normal & 7B & 50.20 & 26.65 & 11.52 & 28.33 \\
\rowcolor{gray!20} Module-of-Thought & 7B & 50.01 & 29.81 & 14.36 & 30.76 \\
\bottomrule
\end{tabular}
\label{tab:dataset}
\end{table*}




==> tables/leetcode.tex <==
\iffalse 
\begin{table*}[t!]
\centering
\caption{\textbf{LeetCode results by \emph{pass@1} (\%).} Competitive approaches include StarCoder~\cite{starcoder}, WizardCoder~\cite{wizardcoder} and CodeLlama series models~\cite{codellama}. } 

% \vspace{-2mm}
\setlength{\tabcolsep}{4.1mm}
\begin{tabular}{lr|ccccccccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Size} & \multicolumn{2}{c}{Easy} & \multicolumn{2}{c}{Medium} & \multicolumn{2}{c}{Hard} & \multicolumn{2}{c}{All} \\
& & Avg & Strict & Avg & Strict & Avg & Strict & Avg & Strict \\
 \midrule
\multirow{3}{*}{CodeLlama}
 & 7B & 27.71 & 15.05& 8.91 & 0.00& 4.54 & 0.00 & 13.72 & 5.02 \\
 & 13B & 29.91 & 12.90& 9.52 & 0.00& 3.19 & 0.00 & 14.21 & 4.30 \\
 & 34B & 36.01 & 20.43& 10.71 & 2.35& 3.33 & 0.00 & 16.68 & 7.59 \\
 \midrule
\multirow{3}{*}{CodeLlama-Python}
 & 7B & 14.70 & 7.53& 5.82 & 0.00& 1.11 & 0.00 & 7.21 & 2.51 \\
 & 13B & 31.44 & 16.13& 8.36 & 0.59& 2.68 & 0.00 & 14.16 & 5.57 \\
 & 34B & 38.68 & 22.58& 12.59 & 2.35& 4.28 & 0.00 & 18.52 & 8.31 \\
 \midrule
\multirow{3}{*}{CodeLlama-Instruct}
 & 7B & 20.18 & 12.90& 5.24 & 0.00& 2.98 & 0.00 & 9.47 & 4.30 \\
 & 13B & 36.15 & 21.51& 13.70 & 1.76& 6.06 & 0.00 & 18.64 & 7.76 \\
 & 34B & 49.37 & 33.33& 14.03 & 2.94& 4.71 & 0.00 & 22.70 & 12.09 \\
\midrule
StarCoder & 15B & 28.83 & 19.35& 9.17 & 1.18& 3.89 & 0.00 & 13.97 & 6.84 \\
WizardCoder & 15B & 49.05 & 31.18& 12.17 & 3.53& 4.38 & 0.00 & 21.87 & 11.57 \\
\midrule
% results train on the single dataset
% \rowcolor{gray!20}MoTCoder & 15B & 52.76 & 46.24& 45.48 & 36.47& 14.57 & 8.54 & 37.60 & 30.41 \\
\rowcolor{gray!20}MoTCoder & 15B & 66.40 & 59.14& 57.41 & 51.76& 24.22 & 19.51 & 49.34 & 43.47 \\
% \midrule
% GPT-3.5 & - & 30.54 & 19.35& 4.90 & 1.76& 3.56 & 0.00 & 13.00 & 7.04 \\
\bottomrule
\end{tabular}
\label{tab:leetcode}
% \vspace{-2mm}
\end{table*}
\fi

==> tables/modular.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% modular inference
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{table*}[t!]
\centering
\caption{\textbf{Experiments of modular ability}. We conducted inference using both normal and modular prompts, as demonstrated in \cref{fig:prompts} and show APPS test results by \emph{pass@1} (\%). Comparable approaches include StarCoder~\cite{starcoder} and WizardCoder~\cite{wizardcoder} with the same size of 15B.}

% \setlength{\tabcolsep}{4mm}
\setlength{\tabcolsep}{6.3mm}
\begin{tabular}{lcc|cccc}
\toprule
Model & Size & Prompt & Introductory & Interview & Competition & All \\
\midrule
\multirow{2}{*}{StarCoder} & \multirow{2}{*}{15B}  & Normal &  7.25 & 6.89 & 4.08 & 6.40 \\
 &  & Modular &    0.59 & 2.87 &  1.00 &  2.04 \\ 
\midrule
\multirow{2}{*}{WizardCoder} & \multirow{2}{*}{15B} & Normal & 26.04 & 4.21 & 0.81 & 7.90 \\
 &  & Modular & 0.39 &  0.46 &  0.66 &  0.81 \\
\midrule 
% results train on the single dataset
\rowcolor{gray!20} & & Normal & \appsinter{} & \appsintro{} & \appscom{} & \appsavg{} \\
\rowcolor{gray!20} \multirow{-2}{*}{MoTCoder} & \multirow{-2}{*}{15B} & Modular & 35.86 & 18.79 & 11.82 & 20.81 \\
\bottomrule
\end{tabular}
\label{tab:apps_modular_test}
\end{table*}
\fi
